Hierarchical Shrinkage: improving the accuracy and interpretability of tree-based methods

Tree-based models such as decision trees and random forests (RF) are a cornerstone of modern machine-learning practice. To mitigate overfitting, trees are typically regularized by a variety of techniques that modify their structure (e.g. pruning). We introduce Hierarchical Shrinkage (HS), a post-hoc algorithm that does not modify the tree structure, and instead regularizes the tree by shrinking the prediction over each node towards the sample means of its ancestors. The amount of shrinkage is controlled by a single regularization parameter and the number of data points in each ancestor. Since HS is a post-hoc method, it is extremely fast, compatible with any tree growing algorithm, and can be used synergistically with other regularization techniques. Extensive experiments over a wide variety of real-world datasets show that HS substantially increases the predictive performance of decision trees, even when used in conjunction with other regularization techniques. Moreover, we find that applying HS to each tree in an RF often improves accuracy, as well as its interpretability by simplifying and stabilizing its decision boundaries and SHAP values. We further explain the success of HS in improving prediction performance by showing its equivalence to ridge regression on a (supervised) basis constructed of decision stumps associated with the internal nodes of a tree. All code and models are released in a full-fledged package available on Github (github.com/csinva/imodels)

==> 02a_background.tex <==
\section{Background and related work}
\label{sec:background}

Recent work by ~\citet{klusowski2021universal} has shown that all of these methods can be related to linear regression. In particular, they showed that each node in the tree can be associated with a binary feature, and the resulting tree model can be recovered by regressing the responses against this node-based representation. We provide a more detailed description of this process in \cref{sec:theory}. \citet{tan2021cautionary} also provided precise generalization bounds for this class of tree models, and showed that the variance term in the $l_2$ risk scales linearly with the number of leaf nodes. This linear dependence of variance on the number of leaf nodes is startling, and provides a theoretical justification of why deep trees suffer from poor generalization performance due to overfitting. 

Shrinkage in linear models via ridge regression \cite{Hoerl70ridge} is a well-established concept to reduce complexity and variance as the degree of freedoms (number of nodes) grows.
Using the linear regression lens of tree-models, we apply ridge regression instead to derive \method, and show that it regularizes the estimate of noisy leaves with few samples by shrinking them towards their parents.  \textcolor{red}{AA: This paragraph needs to be improved significantly... Need to give description of ridge-regression as well.}
%by shrinking estimated regression coefficients to zero.

One work in a similar vein to \methods is BART~\cite{chipman2010bart}, which also regularizes tree estimates by shrinking the value of its leaf nodes to the training average. However, BART must be used during training rather than be applied posthoc, is computationally intensive, and requires the specification of many non-intuitive hyperparameters such as priors on leaf parameters, and tree structure such as maximum depth and probability of splitting.  

Also related are posthoc methods which aim to help understand a black-box model~\cite{lundberg2019explainable,friedman2001greedy,devlin2019disentangled}. We find that the interpretations from these methods can in fact become clearer when applied to a model after applying \method.

==> YS_temp/ENVIRONMENTS.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{remark}[theorem]{Remark}

==> YS_temp/MACROS.tex <==
% Bold symbols

\newcommand{\bl}{\mathbf{l}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\beps}{\boldsymbol{\epsilon}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}

% Common symbols
\newcommand{\R}{\mathbb{R}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\indicator}{\mathbf{1}}
\newcommand{\Var}{\textnormal{Var}}
\newcommand{\Cov}{\textnormal{Cov}}
\newcommand{\KL}{\textnormal{KL}}

% Paired operators
\DeclarePairedDelimiter{\paren}{(}{)}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\abs}{|}{|}
\DeclarePairedDelimiter{\norm}{\|}{\|}
\DeclarePairedDelimiter{\inprod}{\langle}{\rangle}
\DeclarePairedDelimiter{\braces}{\lbrace}{\rbrace}

% Specialized symbols
\newcommand{\data}[1][n]{\mathcal{D}_{#1}}
\newcommand{\semiempirical}[1][n]{\tilde{\mu}_{#1}}
\newcommand{\partition}{\mathfrak{p}}
\newcommand{\collection}{\mathfrak{C}}
\newcommand{\cell}{\mathcal{C}}
\newcommand{\tree}{\mathcal{T}}
\newcommand{\node}{\mathfrak{t}}
\renewcommand{\dim}{d}
\newcommand{\nsamples}{n}
\newcommand{\coordindices}{[\dim]}
\newcommand{\sampindices}{[\nsamples]}
\newcommand{\hypercube}[1][d]{\braces{0,1}^{#1}}
\newcommand{\uniform}{\mu}
\newcommand{\measure}{\nu}
\newcommand{\risk}{\mathcal{R}}
\newcommand{\oraclerisk}{\mathcal{R}^*}
\newcommand{\vol}{\textnormal{Vol}}
\newcommand{\hamball}{B_{H}}
\newcommand{\funcclass}{\mathcal{F}}


% Misc
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
\newcommand{\mybinom}[2]{\Bigl(\begin{array}{@{}c@{}}#1\\#2\end{array}\Bigr)}


% Editing macros
% \newcommand{\comment}[1]{\textcolor{red}{#1}}





==> YS_temp/theory.tex <==
%\documentclass[11pt]{article}
%\usepackage[utf8]{inputenc}
%\usepackage{fullpage}
%\usepackage{amsmath,amssymb,amsthm,mathtools,xcolor,bm,hyperref,graphicx,float}
%\usepackage{import}
%\usepackage[round]{natbib}

%\input{MACROS.tex}
%\input{ENVIRONMENTS.tex}


% Paired operators
%\DeclarePairedDelimiter{\paren}{(}{)}
%\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
%\DeclarePairedDelimiter{\abs}{|}{|}
%\DeclarePairedDelimiter{\norm}{\|}{\|}
%\DeclarePairedDelimiter{\inprod}{\langle}{\rangle}


%\title{Theory for Shrinkage}
%\date{}

%\begin{document}

%\maketitle

%\section{A greedy optimization perspective for CART and SAPS}

%In recent work, \cite{klusowski2021universal} showed how to interpret CART as a greedy optimization procedure. 
%We briefly summarize his argument here. 
%Suppose we have a working tree model $\hat{f}$ and are trying to make the next split. The weighted impurity decrease $N_n(t)\hat{\Delta}(s)$ for a candidate split $s$ can be computed to be equal to the squared dot product between the residuals of the working model $r^{(i)} \coloneqq y^{(i)} - \hat{f}(\bx^{(i)})$, and the vector of values
%$$
%\psi(s)^{(i)} \coloneqq \frac{\indicator\braces{\bx^{(i)} \in t_L}P(t_R) - \indicator\braces{\bx^{(i)} \in t_R}P(t_L)}{\sqrt{N_n(t)P(t_L)P(t_R)}}.
%$$
%In other words, we have
%\begin{equation} \label{eq:impurity_dec_and_inner_prod}
%    N_n(t)\Delta_{\mathcal{I}}(t) = \inprod{\br, \psi(s)}^2.
%\end{equation}

%Observe that $\psi(s)$ has unit norm, and as such, the impurity decrease is simply the reduction in residual variance from adding the predictor $\psi(s)$ into our regression equation, where the current predictors are the features $\psi(s_1),\ldots,\psi(s_m)$ from each existing split in the working tree, as well as the all ones vector. The tree model predictions are then simply the predictions made by the linear regression on these predictors (see Lemma 3.2 in \cite{klusowski2021universal}.) Furthermore, since reduction in variance is the same so long as the added predictor gives the same eventual linear span, we can replace $\psi(s)$ with the decision stumps
%$$
%\xi(s)^{(i)} \coloneqq \indicator\braces{\bx^{(i)} %\in t_L} - \indicator\braces{\bx^{(i)} \in t_R}.
%$$

%SAPS adds more flexibility to the CART procedure by allowing for a larger search space at each step. The candidate predictors to be added are those $\xi(s)$ associated with candidate splits for each tree in our model, as well as those that are associate with a split over the entire covariate space (i.e. we take $t_L = \braces{\bx \colon \bx_k \leq c}$ and $t_R = \braces{\bx \colon \bx_k > c}$ for some feature $k$ and threshold $c$. Again, the predictions from SAPS are those from the linear regression on these predictors.

%\section{Preliminaries}

%\cite{tan2021cautionary} separated CART into two steps in order to better analyze it. We shall do the same with SAPS. Note that given a split $s$, $\xi(s)$ is the vector of values of the function
%\begin{equation} \label{eq:stump_feature}
%    \phi(\bx) \coloneqq \indicator\braces{\bx \in t_L} - \indicator\braces{\bx \in t_R}
%\end{equation}

%on the training set. We can therefore think of SAPS has having two steps
%\begin{enumerate}
%    \item By iteratively choosing the best split, we learn a set of binary engineered features $z_1,\ldots,z_m$, and a map $\Phi \colon \R^n \to \braces{0,1}^p$ such that we have $\Phi(\bx) = \bz$.
%    \item We run least squares on the response vector $\by$ and the transformed training set $\Phi(\data)$, and obtain a regression vector $\hat{\bbeta}$.
%\end{enumerate}

%In order to make the analysis tractable, we shall analyze an \emph{honest} version of SAPS, in which we use a separate sample $\data[n]'$ to perform Step 1 of the algorithm and generate the features $z_1,\ldots,z_m$. This gives us our map $\Phi$, which we then apply to a the training set $\data$ in order to perform Step 2. As with CART Step 1 is more difficult to analyze, so we will consider the following class of models.

%\begin{definition}
%    Let $\Phi\colon \R^d \to \braces{0,1}^p$ be a feature mapping, and suppose $[p] = I_1 =\braces{1}\sqcup I_2 \sqcup \cdots \sqcup I_m$ be a partition of the feature index set such that $\phi_1 \equiv 1$, and for each $j$, $\braces{\phi_k \colon k \in I_j}$ comprises features of the form \eqref{eq:stump_feature} corresponding to all the splits of a single tree.
%    Given a training set $\data$, let $\hat{\bbeta}_n$ be the set of coefficients from regressing the responses against the transformed data $\Phi(\data)$, with the convention that 
%\end{definition}


%\section{Main results}

%\begin{theorem}[Upper bound]




%\end{theorem}

%\section{Helper Lemmas}


%\begin{lemma}[Leave one-out estimated ridge coefficients]
%\label{lem:ridge_leverage_scores}
%The LOO estimated coefficients satisfy 
%\begin{equation*}
%    \bx^{T}_{i}(\hat{\theta}_{\lambda} - \hat{\theta}^{-(i)}_{\lambda}) = \frac{h^{\lambda}_{i}\hat{e}_{i}}{1 - {h^{\lambda}_{i}}}
%\end{equation*}
%\end{lemma}


%\begin{lemma}[Ridge Leverage Score Identity]
%\label{lem:ridge_leverage_identity}
%    Let $\bX$ be any matrix, let $\bx^{(i)}$ be its $i$-th row, and let $h_{ii}$ be its leverage score.
%    Now let $\bX^{(-i)}$ be $\bX$ with its $i$-th row removed.
%    Then we have
%    \begin{equation} \label{eq:lev_score_identity}
%        h_{ii} = \frac{\norm{\bx}_{(\bX^{(-i)T}\bX^{(-i)}+\lambda I)^{-1}}^2}{1 + \norm{\bx}_{(\bX^{(-i)T}\bX^{(-i)}+\lambda I)^{-1}}^2}.
%    \end{equation}

%\end{lemma}

%\begin{lemma}[Population covariance is diagonal]
%\label{lem:population_covariance_diagonal}
%Consider the population level feature, then we have that population covariance matrix $\E\{\bx \bx^T\}$ is diagonal with diagonal entries $P(t)$
%\end{lemma}

%\begin{lemma}[Concentration for covariance matrix]
    
%\end{lemma}

%\begin{lemma}[When does $\mathcal{E}$ hold]
%\label{lem:empty_cell_leverage}
%Let $\mathcal{E}$ be the event that there is at least one point in the cell for a query point $\bx$. Then we have that the leverage score for $\bx$ where $\bX$ contains the test point is: 
%\begin{equation*}
    
%\end{equation*}
    
%\end{lemma}

%\section{Proof details}

%\begin{lemma}[Variance and side lengths] %\label{lem:variance_and_sides}
%    Let $\uniform$ be the uniform measure on $[0,1]^d$. Let $\cell \subset [0,1]^d$ be a cell. Let $f$ be an additive model as in \eqref{eq:additive_model}, and assume that each component function $\phi_j$ is continuously differentiable with $\beta_j \coloneqq \displaystyle{\min_{a_j \leq t \leq b_j}}\abs*{\phi_j'(t)}$, where $a_j$ and $b_j$ are the lower and upper limits respectively of $\cell$ with respect to coordinate $j$. Then we have
%    \begin{equation} \label{eq:variance_and_sides}
%        \Var_\mu\braces*{f(\bx)~|~\bx \in \cell} \geq \frac{1}{6}\sum_{j=1}^d \beta_j^2(b_j-a_j)^2.
%    \end{equation}
%\end{lemma}

%\begin{proof}
%    Note that $\phi_1(x_1), \ldots, \phi(x_j)$ are independent given the uniform distribution on $\cell$. As such, we have
%    $$
%    \Var\braces*{f(\bx)~|~\bx \in \cell} = \sum_{j=1}^d \Var\braces*{\phi_j(x_j)~|~\bx \in \cell}.
%    $$
%    We can then further write
%    $$
%    \Var\braces*{\phi_j(x_j)~|~\bx \in \cell} = \frac{1}{2}\E\braces*{\paren*{\phi_j(t) - \phi_j(t')}^2}
%    $$
%    where $t, t'$ are independent random variables drawn uniformly from $[a_j,b_j]$. For fixed $t$, $t'$, we use the mean value theorem together with our lower bound on $|\phi_j'|$ to write
%    $$
%    \paren*{\phi_j(t) - \phi_j(t')}^2 = \phi_j'(\tilde{t})^2 \paren*{t-t'}^2 \geq \beta_j^2 \paren*{t-t'}^2.
%    $$
%    Since the expectation of the right hand side satisfies
%    $$
%    \E\braces*{\beta_j^2 \paren*{t-t'}^2} = \frac{\beta_j^2(b_j-a_j)^2}{6},
%    $$
    %we immediately obtain %\eqref{eq:variance_and_sides}.
%\end{proof}

%\bibliography{rf}
%\bibliographystyle{plainnat}

%\end{document}

==> figs/data_classification.tex <==
\begin{tabular}{lrr}
\toprule
                                         Name &  Samples &  Features \\
\midrule
                                        
                                        Heart &      270 &        15 \\
                                Breast cancer &      277 &        17 \\
                                     Haberman &      306 &         3  \\
Ionosphere \cite{sigillito1989classification} &      351 &        34  \\
               Diabetes \cite{smith1988using} &      768 &         8 \\
                                German credit &     1000 &        20  \\
           Juvenile \cite{osofsky1997effects} &     3640 &       286  \\
                                   Recidivism &     6172 &        20 \\
\bottomrule
\end{tabular}

%\begin{tabular}{lrr}
%\toprule
%                                         Name &  Samples &  Features \\
%\midrule
%Ionosphere \cite{sigillito1989classification} &      351 &        34 \\
%               Diabetes \cite{smith1988using} &      768 &         8 \\
%                                German credit &     1000 &        20 \\
%           Juvenile \cite{osofsky1997effects} &     3640 &       286 \\
%                                   Recidivism &     6172 &        20 \\
%             Credit \cite{yeh2009comparisons} &    30000 &        33 \\
%                                  Readmission &   101763 &       150 \\
%\bottomrule
%\end{tabular}


==> figs/data_regr.tex <==
\begin{tabular}{lrr}
\toprule
                                     Name &  Samples &  Features  \\
\midrule
    Friedman1 \cite{friedman1991multivariate} &      200 &        10  \\
    Friedman3 \cite{friedman1991multivariate} &      200 &         4 \\
    Diabetes  \cite{efron2004least} &      442 &        10  \\
    Geographical music &     1059 &       117 \\
    Red wine &     1599 &        11 \\
    Abalone \cite{nash1994population} &     4177 &         8  \\
    Satellite image \cite{romano2020pmlb} &     6435 &        36  \\
    California housing \cite{pace1997sparse} &    20640 &         8  \\


\bottomrule
\end{tabular}
